On Fairness in Committee-based Blockchains

Committee-based blockchains are among the most popular alternatives of proof-of-work based blockchains, such as Bitcoin. They provide strong consistency (no fork) under classical assumptions, and avoid using energy-consuming mechanisms to add new blocks in the blockchain. For each block, these blockchains use a committee that executes Byzantine-fault tolerant distributed consensus to decide the next block they will add in the blockchain. Unlike Bitcoin, where there is only one creator per block with high probability, in committee-based blockchain any block is cooperatively created. In order to incentivize committee members to participate to the creation of new blocks rewarding schemes have to be designed. In this paper, we study the fairness of rewarding in committee-based blockchains and we provide necessary and sufficient conditions on the system communication under which it is possible to have a fair reward mechanism.

==> algorithm_consensus.tex <==
% !TeX root = main.tex

	L'algorithme de consensus unique a pour objectif de permettre aux validateurs, de produire un bloc.
	Les validateurs sont sélectionnés de manière déterministe
	%et en round-Robin 
	par rapport à l'histoire de la Blockchain.
%	Les validateurs de cette hauteur sont les seuls processus à exécuter cet algorithme.
	Pour une hauteur donnée, l'algorithme pour le consensus unique se déroule en \emph{tour}s, et chaque tour a un proposeur choisi par round-robin.
%	Un tour consiste en des échanges entre les validateurs afin de décider un bloc. Si les échanges ne permettent pas de produire le bloc proposé, alors les validateurs passent au tour suivant, et ainsi de suite, jusqu'à décision.	
	Un tour se décompose en 3 phases: PROPOSE, PREVOTE, et PRECOMMIT. %(i) la phase PROPOSE, où un validateur, le proposeur du tour diffuse un bloc, la proposition, (ii) la phase de PREVOTE, où les validateurs diffusent leur prévote dépendamment de ce qu'ils ont distribué concernant la proposition, et (iii) la phase de PRECOMMIT, où les validateurs diffusent leur précommit, dépendamment du nombre de prévotes qu'ils ont distribué pour une même valeur pendant la phase de PREVOTE.
%	
	Chaque phase à une durée maximale qui peut être augmentée dans certaines cas, cela pour garantir la propriété de terminaison.
Quand un processus ne reçoit pas \emph{suffisamment} de messages lors d'une phase (la proposition dans la phase PROPOSE, $2n/3+1$ de prévotes dans la phase PREVOTE, $2n/3+1$ de précommits dans la phase PRECOMMIT) et que le chronomètre correspondant à la phase expire, le processus augmente la durée de ce chronomètre pour le tour suivant.
	
	Quand un validateur reçoit au moins $2n/3+1$ prévotes pour un bloc $B$ pour le tour $r$, nous disons que ce validateur a un \emph{polc}.
%	Nous disons qu'un validateur a un \emph{polc} pour un bloc $B$ à un tour $r$ s'il a reçu au moins $2n/3$ prévotes pour $B$ pour le tour $r$. %quand il était en phase PREVOTE du tour $r$.
%	A \emph{\emph{polc}-Round} (\emph{polc}R) is a tour such that there was a \emph{polc} for a block at tour \emph{polc}R.
Quand un validateur reçoit plus de $2n/3+1$ prévotes pour un bloc $B$ durant un tour $r$, il se \emph{verrouille} sur $B$ au tour de \emph{verrou} $r$: cela signifie qu'il y a au moins $n/3+1$ processus corrects qui ont accepté $B$. 
Un processus verrouillé sur un bloc $B$ pendant un tour $r$, peut se déverrouiller s'il a un \emph{polc} pour un bloc $B' \neq B$ pour un tour $r' > r$. Lorsqu'un processus reçoit un nouveau message, il le diffuse aux autres. 
%
Quand un validateur reçoit au moins $2n/3+1$ précommits de différents processus pour la même valeur $B$ pour un même tour, ce processus \textbf{décide} $B$ et termine. % son exécution de l'algorithme.

Notre analyse nous a permis de trouver quelques bugs, que nous avons corrigés afin de prouver la correction du protocole. En effet, l'algorithme décrit dans Tendermint, présente quelques bugs qui violent entre autre la propriété d'\emph{accord}. De plus une hypothèse supplémentaire est nécessaire pour garantir la \emph{terminaison}.
\begin{enumerate}
	\item Phase PROPOSE:
		Un validateur est le proposeur du tour. %Le proposeur existe, car la liste des validateurs est ordonné, et le proposeur est choisi en tour-robin.
		Le proposeur du tour propose son bloc selon son état. S'il est verrouillé sur une valeur $B$, alors il propose et diffuse $B$ et le tour de verrou.
		%Sinon il attend la proposition du proposeur, et augmente son chronomètre s'il n'a pas distribué la proposition avant la fin du chronomètre actuel. 
		%Puis va à la phase PREVOTE.
	
	\item Phase PREVOTE:
		Le validateur vérifie la validité de la proposition reçue. %, ou non.
		Si (i) le validateur n'est pas verrouillé et que la proposition est valide, ou (ii) le validateur reçoit comme proposition le bloc sur lequel il est verrouillé, ou (iii) la proposition contient un bloc qui a reçu un \emph{polc} plus récemment que le tour de verrou du processus (déverrouillage), alors il diffuse son prévote pour la proposition, sinon il diffuse un prévote pour la valeur par défaut $\nil$.
		Puis attend l'expiration du chronomètre ou la réception d'au moins $2n/3+1$ prevotes de différents validateurs, puis passe à la phase PRECOMMIT. %Si le chronomètre a expiré, il est augmenté pour le tour suivant.
		
	\item Phase PRECOMMIT:
		Si le processus a reçu un \emph{polc} pour un bloc $B$, alors il se verrouille sur $B$, met à jour le jour le tour de verrou, et diffuse son précommit pour $B$. Sinon il envoie un précommit pour la valeur $\nil$ et attend de recevoir au moins $2n/3$ précommit, ou l'expiration du chronomètre, puis passe au tour suivant. %Si le chronomètre a expiré, il est augmenté pour le tour suivant.
\end{enumerate}
%

%
%De part notre analyse, nous nous sommes rendu compte que le protocole avait besoin de quelques légères modifications pour implémenter le consensus. %De plus Tendermint à besoin d'une hypothèse supplémentaire nécessaire, indiquée dans la Section \ref{sec:resultats}, pour satisfaire la \emph{terminaison}.

==> consensus.tex <==
% !TeX root = main.tex

The consensus specification is defined as follows:
	(i) \emph{Termination}, every correct process eventually decides some value; 
	(ii) \emph{Integrity}, no correct process decides twice; 
	(iii) \emph{Agreement}, if there is a correct process that decides a value $v$, then eventually all the correct processes decide $v$; 
	(iv) \emph{Validity}, a decided value is valid, it satisfies a predefined predicate.
	This concept of validity is called external validity. The external validity was introduced by Cachin \emph{et al.} \cite{CKPS01} and has been adapted to blockchains by Crain \emph{et al.}\cite{redbelly17}.

==> fairness.tex <==
% !TeX root = main.tex


\paragraph{Chain quality and Committee-based Blockchains}
	In the blockchain literature, chain quality has been define by \cite{GarayKL15}, and extended by \cite{PS17}, to study fairness in Bitcoin-like systems.
	A blockchain system has the property of chain quality if the proportion of blocks produced by honest processes in any given window, 
	is proportional to their relative mining power. 
	Intuitively, chain quality ensure that malicious processes do not produce more blocks than in expectation, given their mining power.
	One of the difference between Bitcoin-like system and the committee-based blockchains is that in the first, one process produces a block, whereas in committee-based blockchain, a committee (a set) of processes produces a block. 
	A committee is not necessary composed only of correct processes, but can contain Byzantines or correct (with a correctness hypothesis of having some majority of members following the protocol).	
%Recently Pass and Shi defined the fairness of a Proof-of-Work based blockchain protocol for a system of $n$ processes as follows (please refer to \cite{PS17} for the formal definition): 
%	\emph{A blockchain protocol is fair if honest process that wield $\phi$ fraction of the computational resources will reap at least $\phi$ fraction of the blocks in any sufficiently long window of the chain}, where the computational resources represent the merit of the process.
We cannot apply the definition of chain quality to committee-based blockchain.
Instead of defining the fairness with the blocks, we will define it relative to the proportion of total rewards a process gets.


%Informally, we say that a blockchain protocol is fair if any correct process that wield $\phi$ of the total merit in the system will get at least $\phi$ of the total reward that is given in the system.
%	To do so, we examine the structure of a committee-based blockchain, where two mechanism are at play, the \emph{selection} (lines 4), and the \emph{reward} (line 18), and we define fairness relative to those mechanisms.

Informally, we say that a blockchain protocol is fair if any \emph{correct process} (a process that followed the protocol) that wield $\alpha$ fraction of the total merit in the system will get at least $\alpha$ fraction of the total reward that is given in the system. 
In order to tackle the fairness of a committee-based blockchain protocol such as HotStuff, Hyperledger, Redbelly, SBFT or Tendermint, we split the mechanism into two: the \emph{selection mechanism} and the \emph{reward mechanism}. 
The \emph{selection mechanism} selects for each new height the \emph{committee members} (the processes that will run the consensus instance) for that height taking into account the merit of each  process. 
The \emph{reward mechanism}, in charge to distribute rewards to committee members that produce a new block. 
Informally, if the selection mechanism is fair, then each process will become committee member proportionally to its merit; 
and if the reward mechanism is fair then for each height, only the correct committee members get a reward. 
By combining the two mechanisms, a correct process is rewarded at least a number proportional to its merit parameter. %, since the faulty processes do not get any reward.
	
\subsection{Selection Mechanism}
	\subsubsection{Definition and Fairness of Selection Mechanisms}
	
	In a system where the size of the committee is strictly lower than the size of the processes in the system, there should be a way to
	select the members of the committees.
	Always selecting the same processes is a way to centralize the system. That set of selected processes is then the \emph{trusted third-party} blockchain systems aim to avoid.
	
	Formally, a selection mechanism is the function $\selection: \Blocks^{+}\times \mathbb{N} \to \Pi^{n}\times \emptyset$, 
	where $n$ is the size of committees, and $\Blocks^{+}$ represents the set of non-empty blockchains such that 
		\[\selection(\bc,h) = \left\{\begin{array}{r r}
				V_h, 		&\text{if } \bc \text{ is a blockchain and } |\bc|\ge h-1\\
				\emptyset,	&\text{otherwise}\\
			\end{array}\right. .
		\]
		
	In the blockchain, some information can be saved, for instance the stakes of each process that represents their wealth.
	The selection mechanism can select, for instance, processes with the highest stakes, or processes with the lowest stakes,
	or always the same set of processes, or processes that were committee members less often, etc.
	
	To abstract the notion of wealth of a process, we denote by $\alpha_i(t) \in [0,1]$ the merit parameter of $p_i$ at time $t$ 
	proportionally to the total merit at time $t$. Such that $\forall i\in \Pi_\rho, \forall t, \alpha_i(t)$ can be computed with the
	information in the blockchain. 
	Note that this means that merit can be computed with the information inside the blockchain\footnote{Knowing the merit
	of processes excludes this definition to apply to proof-of-work based blockchains, since the mining power in proof-of-work is not known
	in advance.}.
	
	If $\forall t \in \mathbb{N}, \forall i, \alpha_i(t) = \alpha_i(0)$, we denote by $\alpha_i$ the merit of the process $p_i$.
	That means that the merits do not depend on the evolution of the blockchain.
	Let $v_i$ be the number of time $p_i$ becomes committee member, proportionally to the number of blocks, so $v_i \in [0,1]$.
	We propose the following definition of fairness of selection mechanisms where merit are fixed and do not change with time. 
	The definition allows all processes with positive merit to be member of committees infinitely often, 
	and by doing so, respecting their merit.
	
	\begin{definition}[Fairness of Selection Mechanism]
		Assume that the blockchain is built infinitely, so $\forall h\ge0$, there is a block at position $h$.
		We say that a selection mechanism is fair if it respects the following properties:
		\begin{enumerate}
			\item\label{selection1} If $\alpha_i \neq 0$ then $v_i \neq 0$; or equivalently, $\alpha_i \neq 0 \implies \forall h\ge 0, \exists h'\ge h: p_i \in V_{h'}$
			\item\label{selection2} If $\alpha_i \ge \alpha_j$ then $v_i \ge v_j$.
		\end{enumerate}
	\end{definition}
	Informally, condition \ref{selection1} means that each process with a positive merit parameter should become a committee member infinitely often.
	Condition \ref{selection2} means that a process with a low merit cannot be selected more than a process with a higher merit.
	
	A definition of fairness of a generic selection mechanism is still an open question, 
	but such definition should encapsulate the above definition as special case.
	
	\begin{remark}\label{r:selectAll}
		When the size of the committee is exactly equal to the number of processes of the system, the selection mechanism
		is the mechanism always selecting all, which is trivially fair, although not scalable.
	\end{remark}
	%	Proposing a fair selection mechanism is always an open problem, and is out of the scope of this paper.

	\subsubsection{Examples of Selection Mechanisms}
	
	We examine few selection mechanism, based on stakes.
	For instance the selection mechanism that always picks the processes with most stakes is not fair. 
	Since it may select the less wealthy process only a finite time, no matter their merit.
	
	\paragraph{Select the processes with the highest stake.}
%		\begin{figure}[t!]
%			\includegraphics[width=\linewidth]{./Graphique/BarRiche}
%			\caption{Number of selections of process over 100 blocks, when the richest are selected}
%			\label{fig:rich}
%		\end{figure}
		
		\begin{figure}[t!]
		\begin{subfigure}[t]{\textwidth}
			\centering
				\includegraphics[width=\linewidth]{./Graphique/BarRiche}
			\caption{5 000 blocks, Processes with highest stakes are selected}
			\label{fig:rich}
		\end{subfigure}\hfill
		\begin{subfigure}[t]{1\textwidth}
			\centering
				\includegraphics[width=\linewidth]{./Graphique/BarPauvre}
			\caption{10 000 blocks, Processes with lowest stakes are selected}
			\label{fig:poor}
		\end{subfigure}
		\caption{Number of selections of processes}\label{fig:selection}
	\end{figure}
		
		In $\Figure$ \ref{fig:rich}, we consider a system composed of $170$ processes. The committees size is $50$, and
		processes with the highest stakes are the one selected. We run the execution over 5 000 blocks.
		As shown in $\Figure$ \ref{fig:rich}, for the whole execution, only a subset of $50$ processes have been selected
		for the construction of the blockchain.
		Even if that may satisfy certain merits, the more stakes a process has at the beginning, the more merit it has,
		this selection mechanism can be fair only if the processes with non-nil merit are exactly the wealthiest and are all selected in each committee.
		If a process with a non-nil merit is selected only finitely, that violates condition \ref{selection1}; exactly the same subset of processes will be selected, since they are they only rewarded, and that subset should cover all process with a non-nil merit.
	
	\paragraph{Select the processes with lowest stake}
		
%		\begin{figure}[t!]
%			\includegraphics[width=\linewidth]{./Graphique/SelectionPauvre}
%			\caption{Number of selections of process over 100 blocks, when the poorest are selected}
%			\label{fig:poor}
%		\end{figure}
		
		In $\Figure$ \ref{fig:poor}, we consider a system composed of $170$ processes. The committees size is $50$, and
		processes with the highest stakes are the one selected. We run the execution over 10 000 blocks.
		As shown in $\Figure$ \ref{fig:poor}, processes seems to be selected almost the same number of time,
		which is $2941 \approx 10 000*50/170$.
%		We can see that some processes are at least selected a bit more than others.
%		That can be explained by the two first blocks.
		This mechanism is fair according to when all the processes have the same merit; this is a way to achieve
		egalitarianism studied in \cite{KKNZ19}, which means that all processes have the exact same opportunity to get a reward.
		Another way to achieve egalitarianism is to selected processes with the lowest number of selection.
%		, as shown in $\Figure$ \ref{fig:lessSelected}.
		
		
		\begin{remark}\label{r:importanceFairnessSelection}
			An unfair selection mechanism can lead to a centralization of the system, by always letting the same processes decide the next block.
			Although the assumption of bound on Byzantine processes does not depend on the selection mechanism, we note that
			when a selection mechanism selected the processes with the lowest stakes, and only correct processes in committees are rewarded,
			at some point processes that were non-correct will have the least stake, and thus be selected. Mechanisms using the number of
			selections seem not to have that issue.
		\end{remark}
	
\subsection{Reward Mechanism}\label{ssec:rewmech}
	\subsubsection{Definition of Reward Mechanism}
		In blockchain systems, process that produces and adds blocks to the blockchain are rewarded.
		In a committee-based blockchains, a committee is the producer of the block.
		Within that committee, some processes may not behave as prescribed.
		There may be different ways of rewarding members of committees.
		To do so, we define what we call a \emph{reward mechanism}. A reward mechanism consists of the reward function defined as follow:
		$\reward: \Blocks^{+}\times \mathcal{P}(\textit{Information}) \times \mathbb{N} \to \mathbb{R}^{|\Pi|}\times (\bot, \dots, \bot)$,
		where $\mathcal{P}(\textit{Information})$ is the power set of all messages, and $\textit{Time}$ represents
		the set of times.
		
		If $\bc$ is a blockchain and $|\bc|< h$, $\reward(\bc,\info,h) = (\bot, \dots, \bot)$.
		Otherwise, it assigns to each process a given reward, null or not.
%		\[\reward(\bc,\info,h) = \left\{\begin{array}{r l}
%				(\bot, \dots, \bot), 		&\text{if } \bc \text{ is a blockchain and } t, |\bc|< h\\
%				(r_1^h, \dots, r_k^h),	&\text{otherwise, where $k$ is the total number of processes}\\
%			\end{array}\right. ,
%		\]
		In $\reward(\bc,\info,h)$, $\info$ represents the set of messages received, $h$ the height of the blockchain $\bc$ 
		where the reward of committee member is computed.
		
		A reward is considered distributed if it is written in the blockchain. 
		The second part of the reward mechanism is to choose when to
		distribute the rewards corresponding for a given height.
		We consider that for each production of block its rewards are distributed in one block and not over different blocks, 
		such that after the distribution of rewards
		a process know if it has been rewarded or not.
		Note that once rewards are distributed, they cannot change any more.
%%%%%		We denote by $r_i^h$ the reward process $p_i$ got for the height $h$.
		Some blockchains system adds a system of punishment, called \emph{slashing}, 
		to remove, afterwards, some rewards a process has if there is a proof of some misbehaviours.
		
		
%		\paragraph{How it works ?} \textcolor{red}{Is it needed to explain more how a reward is written in the blockhain ?}
	\subsubsection{Fairness of Reward Mechanism}
		We define the following properties for characterizing the fairness of a reward mechanism. 
		Let $h$ be a height. 
		Recall that $p_i$ is considered $h$-correct if during the period of height $h$, $p_i$ followed the protocol.
		Each committee member has a boolean variable $r_i^h$, which we call \emph{reward parameter} defined as follow:
		\begin{enumerate}
%%%%%%%	This condition is for forkable blockchains
%%			\item If a block is not in the blockchain, committee member that produced that block should not be rewarded for it.
%%%%%%%
%			\item \label{fairness1} For each block in the blockchain, all  correct committee members for that block have a reward parameter  for that block greater than $0$,
			\item \label{fairness1} If $p_i$ is a not a committee members for $h$, then $r_i^h=0$,
			\item \label{fairness2} \textbf{$h$-completeness.} If $p_i$ is a committee members for $h$ and $p_i$ is $h$-correct, then $r_i^h=1$,
			\item \label{fairness3} \textbf{$h$-accuracy.} If $p_i$ is a committee members for $h$ and $p_i$ is not $h$-correct, then $r_i^h=0$.
			
%			\item \label{fairness2} For each block in the blockchain, all faulty committee members and the processes that are not committee members should have a reward parameter  for that block equal to $0$.

%			\item \label{fairness4} A process gets a reward for a block if and only if it has a reward parameter for that block greater than $0$.
%			\Pitem \label{fairness4bis} There exists a height $h$ such that for a block in the blockchain at   height $h' > h$ a process gets a reward for that block if and only if it has a reward parameter for that block greater than $0$.

		%	\item If a process $p_i$ has more \emph{merit} than a process $p_j$, then $p_j$ cannot get more reward than $p_i$.
		\end{enumerate}
		%\begin{enumerate}[4'.]
		%	\item \label{fairness4bis} There exists a height $h$ such that for all block in the blockchain at a height $h' > h$ a process gets a reward for that block if and only if it has a merit parameter for that block greater than $0$.
		%\end{enumerate}
		If $r_i^h=0$, it means that $p_i$ is not rewarded for height $h$, and if $r_i^h=1$, $p_i$ has been rewarded for $h$.
		The properties are analogous to properties of failure detectors.
		
		\begin{remark}
			Note that we do not reward non-committee members. 
			In this article, we do not consider delegations. When a process delegates to a committee member, 
			once the committee member is rewarded, all of its delegates are rewarded proportionally to what they delegatied.
			In future works, we may consider the case of committee-based blockchains with delegations. 
			To do so, reward parameter must contains more information and not just a boolean variable.
		\end{remark}
		
		Let $\mathcal{R}$ be a reward mechanism. 
		\begin{definition}[Complete Fairness of a Reward Mechanism]
			If $\forall h>0$, $\mathcal{R}$ satisfies conditions \ref{fairness1} and $h$-completeness (condition \ref{fairness2}),
			we say that $\mathcal{R}$ satisfies complete fairness.
		\end{definition}
		If a reward mechanism satisfies complete fairness, it means that for all height $h>0$, 
		all $h$-correct committee members are rewarded, and non-committee members are not. 
		% , thanks to condition \ref{fairness1}, and all $h$-correct committee members get a reward \ref{fairness2}, thanks to condition \ref{fairness2}.
		
		\begin{proposition}\label{prop:completeFairness}
			There always exists at least one reward mechanism satisfying complete fairness. 
		\end{proposition}
		Once a block is in the chain, 
		rewarding all committee members, in the next block, for that block and only them,  satisfy conditions \ref{fairness1} and \ref{fairness2}.
		Condition \ref{fairness1} is satisfied since for all height, non-committee members are not rewarded. 
		Condition \ref{fairness2} also holds, for any given height $h$, all committee members of $h$ are rewarded, 
		in particular all $h$-correct committee members.
		
		
		\begin{definition}[Accurate Fairness of a Reward Mechanism]
			If $\forall h>0$, $\mathcal{R}$ satisfies conditions \ref{fairness1} and $h$-accuracy (condition \ref{fairness3}),
			we say that $\mathcal{R}$ satisfies accurate fairness.
		\end{definition}
		If a reward mechanism satisfies accurate fairness, it means that for all height $h>0$, all non $h$-correct committee members are not rewarded. 
		%, thanks to condition \ref{fairness1}, and all $h$-correct committee members get a reward \ref{fairness2}, thanks to condition \ref{fairness2}.
		
		\begin{proposition}\label{prop:accurateFairness}
		There always exists at least one reward mechanism satisfying accurate fairness. 
		\end{proposition}
		Never distributes rewards satisfies conditions \ref{fairness1} and \ref{fairness3}.
		Condition \ref{fairness1} is satisfied since non-committee members are not rewarded.
		Condition \ref{fairness3} holds, since no process is rewarded. 
		In particular for any given height $h>0$, 
		no non $h$-correct committee members is rewarded.
		
		Although simple and trivial to satisfy either complete fairness or accurate fairness, 
		satisfying both at the same time is more complex and not always possible.
		
		\begin{definition}[Fairness of a Reward Mechanism]
			If $\forall h>0$, $\mathcal{R}$ satisfies conditions \ref{fairness1}, $h$-completeness (condition \ref{fairness2}) and $h$-accuracy (condition \ref{fairness3}),
			we say that $\mathcal{R}$ is fair.
		\end{definition}
		
		We say that a reward mechanism is fair when at each height $h$, all and only $h$-correct committee members are rewarded.
		
		
		\begin{theorem}\label{t:strongFairness}
			There exists a fair reward mechanism in a committee-based blockchain protocol iff the system is synchronous.
		\end{theorem}
		\begin{proofT}%[Proof of Theorem \ref{t:strongFairness}]
			We prove this theorem by double implication.
			\begin{itemize}
				\item If there exists a fair reward mechanism, then the system is synchronous.
				
					Let $\mathcal{R}$ be a reward mechanism. By contradiction, we assume that $\mathcal{R}$ is fair and that the system is not synchronous. 
					
					$V_{h}$ is the set of committee members for the height $h$. Let $k>0$ be the number of blocks to wait before distributing the rewards for $V_h$. The reward is given by the committee $V_{h'}$, where $h'=h+k$.
					Since the system is not synchronous, the committee members of height $h'$, $V_{h'}$, may not receive all messages from $V_{h}$ before distributing the rewards.
					
					By conditions \ref{fairness1}, and \ref{fairness2}, 
					Since the reward mechanism is fair, by conditions \ref{fairness1} - \ref{fairness3},
					all and only the $h$-correct committee members of the height $h$ have a reward parameter equal to $1$.
					That means that the $h'$-correct committee members of $V_{h'}$ know exactly 
					who were the $h$-correct committee members in $V_h$,
					they got all the messages before giving the reward. Contradiction, so the system is synchronous.
					
				\item If the system is synchronous, then there exists a fair reward mechanism.
					
					We assume that the system is synchronous and $\forall h>1$, all messages sent by $h$-correct processes at height $h$ are delivered before the block at height $h+1$. 
					Let $\mathcal{R}$ be the following reward mechanism:
					Let $h$ be a height. Rewards for a block at height $h$ are distributed at height $h+1$  by the committee $V_{h+1}$.
					\begin{itemize}
						\item If a process is not a committee member for height $h$, 
							set its reward parameter to $0$, this is known since processes are already at height $h+1$.
						\item By combining the messages from committee member of $h$ processes, since the communication system is synchronous, it is possible to differentiate between $h$-correct and non $h$-correct committee members, and so set the reward parameter of $h$-correct committee members of $h$ to $1$; and set the reward parameter of non $h$-correct committee members of $h$ to $0$.
					\end{itemize}
%					We just proved that $\mathcal{R}$ is fair.
%					
%					Note that the system is synchronous and messages sent are delivered within at most $x$ blocks.
%					Therefore, the exact set of correct validators at $H-x$ is known by all at $H$. 
					By construction, the committee members in $h+1$ give rewards to all and only $h$-correct committee members, so $\mathcal{R}$ is fair, because it satisfies all fairness conditions \ref{fairness1} - \ref{fairness3}.
			\end{itemize}
%			\begin{itemize}
%				\item If the system is synchronous, then there exists a fair reward mechanism.
%					
%					We assume that the system is synchronous and all messages are delivered before the $x$ following blocks. We consider the following reward mechanism.
%					For all the correct validators at any height $H$, if $H-x \le 0$, do not reward yet, otherwise:
%					\begin{itemize}
%						\item Set to $1$ the reward parameters of all correct validators in $H-x$, and to $0$ the merit parameters of the others.
%						\item Reward only the validators with a reward parameter equal to $1$ from the height $H-x$.
%					\end{itemize}
%					We prove in the following that the above reward mechanism is fair.
%					
%					Note that the system is synchronous and messages sent are delivered within at most $x$ blocks.
%					Therefore, the exact set of correct validators at $H-x$ is known by all at $H$. 
%					By construction, the validators in $H$ exactly give the reward to the correct validators who are the only one with a reward parameter for $H-x$ greater than $0$, which satisfies the fairness conditions (\ref{fairness1}, \ref{fairness2} and \ref{fairness3}.
%				\item If there exists a fair reward mechanism, then the system is synchronous.
%					
%					By contradiction, we assume that $\mathcal{P}$ is a protocol having a fair reward mechanism and that, the system is not synchronous.
%					We say that the validators following $\mathcal{P}$ are the correct validators.
%					Let $V^{i}$ be a set of validators for the height $i$, and $V^{j}, (j >i)$ be the set of validators who gave the reward to the correct validators in $V^i$. 
%					Since the system is not synchronous, the validators in $V^{j}$ may not receive all messages from $V^{i}$ before giving the reward.
%					
%					By conditions \ref{fairness1}, and \ref{fairness2}, 
%					it follows that all and only the correct validators in $V^i$ have a reward parameter greater than $0$.
%					Since the reward mechanism is fair, with the condition \ref{fairness4}, we have the validators in $V^{j}$ gave the reward only to the correct validators in $V^i$. That means that the correct validators in $V^j$ know exactly who were the correct validators in $V^i$,
%					so they got all the messages before giving the reward. Contradiction, which conclude the proof.
%			\end{itemize}
			\renewcommand{\toto}{t:strongFairness}
		\end{proofT}
		
		If there is no synchrony, then there cannot be a fair reward mechanism for committee-based blockchains. 
		Our definition of fairness states that for any height conditions \ref{fairness1}-\ref{fairness3} are satisfied. 
		At any time, processes receive all rewards they deserve.
		This definition can be weaken.
		
		\begin{definition}[Eventual Fairness of a Reward Mechanism]
			If $\exists h_0>0: \forall h \ge h_0$, $\mathcal{R}$ satisfies conditions \ref{fairness1},  $h$-completeness (condition \ref{fairness2}) and $h$-accuracy (condition \ref{fairness3}),
			we say that $\mathcal{R}$ is eventually fair.
		\end{definition}
		
		A reward mechanism is eventually fair if after an unknown time, the rewards are distributed to and only 
		to committee members following the protocol.
		
		We note that if a reward mechanism is fair, then it is eventually fair but the reverse (reciprocal) is not necessarily true.
	
		
		\paragraph{Detectable Byzantine Processes.}
			In synchronous systems, it is always possible to detect Byzantine processes, for example using the broadcast abstraction 
			\emph{detectable all-to-all} (DA2A) defines in \cite{LSKM19}.
			Detecting Byzantine processes allows to not reward them, and then to satisfy condition \ref{fairness3}. 
			In eventual synchronous systems on the other hand, we conjecture that it is not possible to always detect all Byzantine processes
			without counterpart.
			It seems impossible, to differentiate for instance \emph{almost silent} Byzantine processes to slow correct processes,
			or even processes that do not follow the protocol but only sends final values to correct ones.
%			In a case of only committee member, a non $h$-correct committee member 
			We say that a Byzantine is \emph{detectable} if it is possible for correct processes to detect it by combining information
			they have, for example, what they see during the execution. 
			
			In this paper, we do not specify the class of detectable processes, which can be an interesting future work.
		
		\begin{theorem}\label{t:eventualFairness}
			There exists an eventual fair reward mechanism in a committee-based blockchain protocol iff the system is (eventually) synchronous and Byzantine processes are detectable.
		\end{theorem}
		\begin{proofT}%[Proof of Theorem \ref{t:eventualFairness}]
			We prove this theorem by double implication.
			\begin{itemize}
				\item If there exists an eventual fair reward mechanism, then system is eventually synchronous or synchronous and Byzantine processes are detectable.
				
					Let $\mathcal{R}$ be a reward mechanism. By contradiction, we assume that $\mathcal{R}$ is eventually fair and 
					that the system is neither synchronous nor eventually synchronous.
					
					
					If $\mathcal{R}$ is fair, by theorem \ref{t:strongFairness}, the communication is synchronous, which ends the proof.
					Otherwise, since $\mathcal{R}$ is eventually fair, then there is a point in time $h$ from which all the rewards are correctly distributed, so for any height $h'\ge h$ $h'$-correct committee members of committees at height $h'$ are able to distinguish between non-correct processes for the height they are distributing rewards.
					If we consider $h$ as the beginning of the execution, then we have that $\mathcal{R}$ is fair, 
					and by theorem \ref{t:strongFairness}, the message delay is upper bounded.
					We have that after $h'$, the message delay is upper bounded, so the communication is eventually synchronous.
					
				\item If the system is eventually synchronous or synchronous, and Byzantine processes are detectable, then there exists an eventual fair reward mechanism.
					
					If the system is synchronous, the proof follows directly from theorem \ref{t:strongFairness}.
					Consider that the system is eventually synchronous, but not synchronous.
					Let $\mathcal{R}$ be the following mechanism:
					Let $h$ be a height. Rewards for a block at height $h$ are distributed at height $h+1$ by the committee $V_{h+1}$.
					\begin{itemize}
						\item If a process is not a committee member for height $h$, 
							set its reward parameter to $0$, this is known since processes are already at height $h+1$.
						\item By combining the messages from committee member of $h$ processes, if there is not sufficient information to detect the behaviour of processes, reward only those detected as $h$-correct and in $V_h$, and the process proposing the distribution of reward increases the duration to wait before starting the next height ($\Delta$ in $\Figure$ \ref{fig:repConsensus}) .
						If there is enough information to detect the behaviour of all processes in $V_h$, then reward the $h$-correct processes in $V_h$ and do not reward non $h$-correct processes in $V_h$.
					\end{itemize}
					$\mathcal{R}$ is eventually fair.
%					When starting the height $H$, the correct validator for $H$ do the following:
%					\begin{itemize}
%						\item Start the time-out for the reception of the messages from validators for the block $H-1$;
%						\item Wait for receiving the messages from validators for the block $H-1$ or the time-out to expire.
%							If the time-out expires before the reception of more that $2n/3$ of the messages, increase the time-out for the next time;
%						\item Set to $1$ the reward parameters for $H-1$ of the correct validators which messages where received, and to $0$ the merit parameters of the others;
%						\item Reward only the validators for the height $H-1$ which have a merit parameter different than $0$.
%					\end{itemize}
%					Since the system is eventually synchronous, eventually when the system will become synchronous, the processes, in particular the validators for $H$ will receive messages for all the correct validators from round $H-1$ before the round $H$.
%					We note that the condition \ref{fairness4bis} is a weaker form of the condition \ref{fairness4} where we do not consider the beginning.
%					So we end the proof by applying the theorem \ref{t:strongFairness} from the time when the system becomes synchronous.
%					
			\end{itemize}
%			\begin{itemize}
%				\item If the system is eventually synchronous or synchronous, then there exists an eventual fair reward mechanism.
%					
%					If the system is synchronous, the proof follows directly from theorem \ref{t:strongFairness}. Otherwise, we prove that the following reward mechanism is eventually fair.
%					When starting the height $H$, the correct validator for $H$ do the following:
%					\begin{itemize}
%						\item Start the time-out for the reception of the messages from validators for the block $H-1$;
%						\item Wait for receiving the messages from validators for the block $H-1$ or the time-out to expire.
%							If the time-out expires before the reception of more that $2n/3$ of the messages, increase the time-out for the next time;
%						\item Set to $1$ the reward parameters for $H-1$ of the correct validators which messages where received, and to $0$ the merit parameters of the others;
%						\item Reward only the validators for the height $H-1$ which have a merit parameter different than $0$.
%					\end{itemize}
%					Since the system is eventually synchronous, eventually when the system will become synchronous, the processes, in particular the validators for $H$ will receive messages for all the correct validators from round $H-1$ before the round $H$.
%					We note that the condition \ref{fairness4bis} is a weaker form of the condition \ref{fairness4} where we do not consider the beginning.
%					So we end the proof by applying the theorem \ref{t:strongFairness} from the time when the system becomes synchronous.
%					
%				\item If there exists an eventual fair reward mechanism, then system is eventually synchronous or synchronous.
%					
%					If the reward mechanism is fair, by theorem \ref{t:strongFairness}, the communication is synchronous, which ends the proof.
%					Otherwise, since the reward mechanism is eventually fair, then there is a point in time $t$ from when all the rewards are correctly distributed.
%					By considering $t$ as the beginning of our execution, then we have that the reward mechanism is fair after $t$, so by the theorem \ref{t:strongFairness}, the system is synchronous from $t$.
%					If the system were not synchronous before $t$, that means that it is eventually synchronous, otherwise, it is synchronous.
%					Which ends the proof.
%			\end{itemize}
			\renewcommand{\toto}{t:eventualFairness}
		\end{proofT}
		
	
	
	 	\begin{corollary}\label{c:asyncFairness}
			In an asynchronous system, there is no (eventual) fair reward mechanism in a committee-based blockchains tolerating Byzantine processes.
			Note that this result holds even if all the processes are correct, but the protocol tolerates Byzantine processes.
		\end{corollary} 
	
	
%		\begin{definition}[(Eventual) Fairness of a blockchain protocol]
%			A blockchain protocol is \emph{fair} (resp. \emph{eventually fair}) if it has a fair selection mechanism and a fair (resp. eventually fair) reward mechanism.
%		\end{definition}
	
	
		\begin{remark}
			If $|V| > 1$ then for a reward mechanism to be (eventually) fair, the reward cannot be given directly in the block. In fact for any height $h\ge 1$ the set of $h$-correct committee members cannot be known in advance.
			If $|V| = 1$, however, the reward can be directly given to the only committee member, so in the block.
		\end{remark}
		

==> resultats.tex <==
% !TeX root = main.tex

	In this section, we discuss the consequences of the synchrony on the existence of a fair reward in Repeated Consensus based  blockchain protocols where  the blockchain is constructed by a mechanism of repeated consensus. That is,  at each height, a subset of processes called validators produce a block executing an instance of One-Shot Consensus.

==> tendermintFairness.tex <==
% !TeX root = main.tex

	The reward mechanism in Tendermint is as follow:
	
The validators selection mechanism is part of a separate module of Cosmos project  \cite{cosmos}, which has Tendermint as core-blockchain. The selection mechanism is today left configurable by the application, therefore in the following we do not address this part. The  rewarding mechanism, on the other hand, referred as the \textit{Tendermint's reward mechanism}  is part of the original Tendermint protocol and it is reported in Figure \ref{fig:repConsensus} at lines \ref{Commit-wait} and \ref{ComDel-01} - \ref{ComDel-02}. The Tendermint's reward mechanism works  as follows:
	\begin{itemize}
		\item Once a new block is decided for height $H$, processes wait for at most   TimeOutCommit time to collect the decision from the other validators for $H$, and put them in their set $toReward$ (Fig. \ref{fig:repConsensus}, lines \ref{Commit-wait} and \ref{ComDel-01} - \ref{ComDel-02}).
		\item During the consensus at height $H$, let us assume that $p_i$ proposes the block that will get decided in the consensus. $p_i$ proposes to  reward  processes in its set $toReward$ (Fig. \ref{fig:repConsensus}, line \ref{repC:cons}). That is, only the processes from which $p_i$ delivered a commit will get a reward for the block at height $H-1$.

	\end{itemize}
	%In the following, we assume that the \emph{selection mechanism} is fair and study the fairness of the reward mechanism.

%\begin{lemma}\label{l:totalView}
%	%The reward mechanism is fair if and only if there is a \emph{perfect} view of the correct validators.
%	If there is a \emph{perfect} view of the correct validators for all blocks before the rewards is given, then there exists a fair reward mechanism.
%\end{lemma}
%\setcounter{theorem}{11}	
\begin{lemma}\label{l:tendermintNotFair}
		The Tendermint's reward mechanism is not eventually fair.
	\end{lemma}

Let us observe that to make the Tendermint's reward mechanism at least eventually fair it is sufficient to increase $TimeOutCommit$ for each round until it catches up the message delay. We refer to this variant as the \textit{Tendermint's reward mechanism with modulable timeouts.} 
	\begin{lemma}\label{l:tendermintModFair}
		The Tendermint's reward mechanism with modulable timeouts is eventually fair.
	\end{lemma}
	%With the assumption of weakly synchrony, there is a time after which the message transfer delay is upper bounded by some finite $\delta$.
%	If correct processes increase their $TimeOutCommit$ each time they do not deliver all the commit for a height, eventually in the period of synchrony, validators for height $H$ will deliver all message for height $H-1$. At that point, the reward can be distributed fairly for the correct validators for $H-1$.
%	For space limitation, the complete proof of Lemma \ref{l:tendermintModFair} can be found in the Appendix and \cite{ADPT18}. 
	
%	The proof of the next theorem is a direct consequence of Lemma \ref{l:tendermintModFair}.
	\begin{theorem}\label{t:tendermintFair}
		In an eventual synchronous system, if the selection mechanism is fair, then Tendermint Repeated Consensus with the reward mechanism with modulable time-outs, is eventually fair.
	\end{theorem}
